Mapping Partisan Fault Lines Within DAOs

Decentralised Autonomous Organisations (DAO) can fragment when partisan communities emerge within their governance structures, leading to organisational splits known as "forks". We present a method to detect these emerging communities by analysing on-chain voting behaviour before fragmentation occurs. Our approach extracts voting events from governance smart contracts, constructs voter matrices encoding participation patterns, and applies pairwise dissimilarity analysis to quantify voting divergence between addresses. We visualise these relationships using multidimensional scaling and identify partisan communities through k-means clustering with silhouette score optimisation. Using Nouns DAO as a case study, a protocol that has experienced multiple documented forks, we demonstrate that addresses that would later fork cluster together months before actual fragmentation events. Our analysis of 330 proposals spanning from contract deployment to the first major fork shows that 90% of fork addresses cluster together in the final 44 proposals, compared with only 47% in randomised data. These results indicate that partisan communities can be detected and visualised through on-chain governance analysis, providing retrospective evidence of emerging divisions before they cause organisational fragmentation.

==> acronyms.tex <==
\newacronym{dao}{DAO}{Decentralised Autonomous Organisation}
\newacronym{evm}{EVM}{Ethereum Virtual Machine}
\newacronym{mds}{MDS}{multidimensional scaling}
\newacronym{mp}{MP}{Member of Parliament}
\newacronym{nft}{NFT}{non-fungible token}
\newacronym{roi}{RoI}{Republic of Ireland}
\newacronym{rpc}{RPC}{remote procedure call}
\newacronym{setu}{SETU}{South East Technological University}
\newacronym{uk}{UK}{United Kingdom}

